MinT: Boosting Generalization in Mathematical Reasoning via Multi-View Fine-Tuning

Reasoning in mathematical domains remains a significant challenge for relatively small language models (LMs). Many current methods focus on specializing LMs in mathematical reasoning and rely heavily on knowledge distillation from powerful but inefficient large LMs (LLMs). In this work, we explore a new direction that avoids over-reliance on LLM teachers, introducing a multi-view fine-tuning method that efficiently exploits existing mathematical problem datasets with diverse annotation styles. Our approach uniquely considers the various annotation formats as different "views" and leverages them in training the model. By postpending distinct instructions to input questions, models can learn to generate solutions in diverse formats in a flexible manner. Experimental results show that our strategy enables a LLaMA-7B model to outperform prior approaches that utilize knowledge distillation, as well as carefully established baselines. Additionally, the proposed method grants the models promising generalization ability across various views and datasets, and the capability to learn from inaccurate or incomplete noisy data. We hope our multi-view training paradigm could inspire future studies in other machine reasoning domains.

==> evaluation.tex <==
\Section{Evaluation}


\subsection{Datasets}

















\subsection{Baseline}







==> related_work.tex <==

\section{Related Work}

\subsection{Multi-View Learning}
In traditional machine learning, multi-view learning often refers to semi-supervised co-training algorithms~\citep{nigam2000analyzing,sun2011robust}. These algorithms exploit multiple views of data to iteratively learn separate classifiers, each of which provides predicted labels for the unlabeled data of the others, \ie, semi-supervised setting. Another thread of multi-view learning lies in clustering methods. These methods aim to partition the data across multiple views, which provide complementary information to each other, to obtain a more refined representation of the data \citep{bickel2004multi,li2015large,cao2015diversity}.




More recently, the concept of multi-view learning has been extended to deep learning~\citep{song-2020-structural}. For instance, \cite{wang2022multi} employs multiple transformers to learn a comprehensive embedding for speaker recognition. Similarly, \cite{zhong2023knowledge} utilizes views based on context, syntax, and knowledge to analyze the sentiment of sentences. Moreover, \cite{allen2022towards} shows that the multi-view learning strategy can be associated with ensemble learning and knowledge distillation techniques to improve the accuracy of image classification tasks.

While traditional multi-view learning approaches aim to improve data representation through understanding different perspectives, our work takes a different path by focusing on mathematical problem solving, which is unlike deterministic tasks such as image classification or sentiment analysis. This free-form generation task can be characterized by its diverse solution views shown in Table \ref{tab:view_example}. This situation is further complicated by the existence of multiple acceptable solutions for a problem, as discussed in \cite{hong2021learning}. Given these conditions, our goal is not to prioritize any single view, but rather to enhance the accuracy of solutions across all views. In our context, the term ``generalization'' indicates the collaboration and mutual benefit among all the views, differing from the traditional concept of generalizing to a specific view or deterministic task. We hope this work can broaden the application and impact of multi-view learning techniques.

\subsection{Math Word Problem Solving}
Solving math word problems is a common benchmark for evaluating the mathematical reasoning capabilities of NLP models \cite{amini2019mathqa,patel2021nlp,cobbe2021training}. Earlier approaches rely on statistical and rule-based parsing \cite{hosseini2014learning,koncel2015parsing}, then transition to Seq2Seq-based neural networks \cite{xie2019goal,zhang2020graph,jie2022learning}. Recently, Large Language Models (LLMs) have demonstrated success in solving math word problems, surpassing fine-tuned baselines through Chain of Thought (CoT) prompts \cite{wei2022chain,kojima2022large}.

Another thread of research has also explored the distillation of knowledge from LLMs to smaller models \cite{ho2022large, magister2022teaching, shridhar2022distilling, hsieh2023distilling, liang2023let}. These papers primarily leverage LLMs for generating reasoning steps, segmenting problems, or creating customized exercises to train smaller models.

Our research, however, investigates a different approach: using publicly accessible datasets in an efficient way to train effective, smaller LMs for mathematical problem solving. We thus offer a unique perspective, being orthogonal to previous research efforts.



























